Decentralized Infrastructure for Digital Notarizing, Signing and Sharing Files using Blockchain

Traditional paper-based document management has long posed challenges related to security, authenticity, and efficiency. Despite advances in digitalization, official documents remain vulnerable to forgery, loss, and unauthorized access. This thesis proposes a decentralized infrastructure for digital notarization, signing, and sharing of documents using blockchain technology. The research addresses key issues of transparency, immutability, and feasibility by defining system requirements, evaluating existing solutions, and proposing a novel architecture based on distributed systems. By combining cryptographic techniques with decentralized storage, this research contributes to the development of a more secure and efficient framework for managing official documents. The findings highlight the potential of blockchain-based digital notarization to streamline bureaucratic processes, mitigate security risks, and enhance user trust in digital document management.

==> chap2-background-overview/subchapters/blo_5_bl_data_management.tex <==

\subsection{Blockchain Data Management Stack}

As Qian Wei et al. stated in his survey about blockchain data management systems, blockchain systems can be classified in three main categories: standard, hybrid, and DAG (Directed-Acyclic-Graph).

\subsubsection{Standard Blockchain}

A standard blockchain \cite{Hasan2020} system's ledger is a single chain list. The system's transactions are arranged into blocks and confirmed by a mining process. In chronological sequence, the validated blocks are added to the chain. Besides the genesis block, blocks are connected according to their parent block hash in the block header. A transaction block is the fundamental data format of a conventional blockchain system, consisting of a block header and a block content. The block header contains the block metadata, while the block body contains the transactions. The contents of the block header varies slightly amongst blockchain \cite{Haveri2020} systems. These contents may be separated into two groups. The first set contains mining-related information such as timestamp, difficulty, and nonce, while the second contains Merkle root, parent block hash, and block version. A normal blockchain system often uses a file system to store its binary block data and a key-value database to store its metadata for the blockchain storage engine (e.g., Merkle tree and account information). For example, Ethereum stores all of its binary block data as regular files and uses the key-value database LevelDB to store its Merkle tree data, which is used for account verification and querying.

\subsubsection{Hybrid Blockchain}

In contrast to traditional blockchain systems, hybrid \cite{bibitem_13} blockchain systems are not open to all nodes but still provide blockchain benefits such as integrity, transparency, and security. Members of the hybrid blockchain may choose who can participate in the blockchain and whose transactions are public. A hybrid blockchain's blockchain architecture might consist of a single listed chain like a traditional blockchain system or many alliance chains. Because each alliance chain corresponds to a set of ledgers, each peer node in the blockchain \cite{Wang2018} may keep numerous sets of ledgers. Each chain has the same structure as a normal blockchain. A hybrid blockchain system, like a regular blockchain system, stores transactions with the data structure of blocks. Each block consists mostly of three parts: the block's relevant contents, data connected to the preceding block, and block metadata. The block data typically comprises the block hash and account number. The block information mostly consists of the block creation time and signature. Hybrid blockchain often uses a combination of databases and file systems as its blockchain storage engine.

\subsubsection{DAG-based Blockchain}

Tangle is a distributed, decentralized \cite{Vatsaraj2021}, and directed acyclic graph (DAG)-based blockchain architecture. Tangle's DAG-based blockchain organizes all transactions in a DAG instead of grouping them into blocks like Bitcoin and Ethereum do. DAG-based blockchains are not constrained by block generation \cite{Ebejer2012} because they are based on a non-block structure. As a result, DAG-based blockchains offer higher throughput potential and lower latency than block-based blockchains. Each transaction in Tangle is represented by a node in the data structure. Clients issue all transactions through a selective proof-of-work (PoW) process. Tips are transactions that have not been approved by subsequent transactions. The system must select and approve two tips before adding a transaction. A random walking algorithm is used to choose tips for approval during the tip selection process, and a transaction validation algorithm is used to validate transactions along the validation path to prevent double-spending. DAG-based blockchains typically use a relational or key-value database as the blockchain storage engine to store transactions and account information.

In summary, a Standard Blockchain is a chained data structure that links data blocks chronologically. The mining process generates each block, which contains several transactions. The parent block hash in the block header is used to link blocks all the way back to the genesis block. Each allied chain corresponds to a collection of ledgers in the Hybrid Blockchain. As a result, each peer node in the blockchain \cite{10731822} may maintain multiple sets of ledgers, each with the same structure as the traditional blockchain \cite{9642822}.

\begin{figure}[H] % supposedly places it here ...
  \centering
  \includegraphics[width=0.95\linewidth]{chap2-background-overview/images/blockchain_2.png}
  \caption{The Layers of Blockchain Data Management Stack\protect\footnotemark}
  \label{fig:no3}
\end{figure}


\footnotetext{Source: \href{https://arxiv.org/pdf/2111.13683}{A Survey of Blockchain Data Management Systems (https://arxiv.org/pdf/2111.13683)}}

The DAG structure forms the foundation of DAG-based Blockchain. Each node in the graph represents a transaction that points in one direction and eventually connects to a root node. Standard Blockchain is widely used in areas such as digital currency, financial asset transaction settlement, deposit certificates, and anti-counterfeiting data services. Hybrid Blockchain is suitable for scenarios involving multi-organizational information sharing that require transactions both within and outside the organization. DAG-based Blockchain is better suited to the IoT environment, as it practically eliminates transaction costs.

In our case I think the blockchain \cite{8946223} type that would better suit our needs is a hybrid one due to increased security of data retrieval, having the possibility to offer access to certain nodes only to whom it may concern.
